The Principle of Unchanged Optimality in Reinforcement Learning Generalization

Several recent papers have examined generalization in reinforcement learning (RL), by proposing new environments or ways to add noise to existing environments, then benchmarking algorithms and model architectures on those environments. We discuss subtle conceptual properties of RL benchmarks that are not required in supervised learning (SL), and also properties that an RL benchmark should possess. Chief among them is one we call the principle of unchanged optimality: there should exist a single $\pi$ that is optimal across all train and test tasks. In this work, we argue why this principle is important, and ways it can be broken or satisfied due to subtle choices in state representation or model architecture. We conclude by discussing challenges and future lines of research in theoretically analyzing generalization benchmarks.

==> method.tex <==



\section{Notation and Methods}
To formalize our supervised learning analogy to the RL setup, let $\Theta$ be a distribution over parameters $\theta$ that parametrize an MDP family $\{\mathcal{M}_\theta : \theta \in \Theta\}$. Each $\theta$ parametrizes some state space, action space, reward, transitions, and observation function, with $\mathcal{M}_\theta = (\mathcal{S}_\theta, \mathcal{A}_\theta, r_\theta, \mathcal{T}_\theta, S_{0,\theta}, w_{\theta})$. An appropriate train and test set can then be created by randomly sampling $\theta \sim \Theta$ and training or evaluating within $\mathcal{M}_\theta$. 


For sake of notational simplicity, we denote $s$ as the observation rather than $w_{\theta}$. The standard policy gradient \cite{reinforce} without a discount factor where $\tau = (s_{1},a_{1},...,s_{T}, a_{T})$ is the gradient with respect to the true objective:
\begin{equation}\nabla_{\phi} R(\pi_{\phi}) = \E_{\tau} \left[ \left( \sum_{t=1}^{T} r_{t} \right) \left(\sum_{t=1}^{T} \nabla_{\phi}  \log  \pi_{\phi}(a_{t} | s_{t}) \right) \right] \end{equation}
However, a more practical and modern RL algorithm such as PPO \cite{ppo} maximizes the objective $R^{PPO}(\beta) = L^{CLIP}(\phi) - c_{1} L^{VF}(\phi) + c_{2} S(\pi_{\phi})$, where $L^{CLIP}$ is the clipped advantage ratio, $L^{VF}$ is the value function error, and $S$ is entropy.

These surrogate losses inherently affect our definition of the "gradient cosine similarity" (GCS) between training and test gradients and what the GCS measures. With basic policy gradient this is simply the normalized dot product between $\nabla_{\phi} R_{train}(\pi_{\phi}) $ and $\nabla_{\phi}R_{test}(\pi_{\phi})$ which is unbiased, but with algorithms such as PPO, the GCS becomes biased. On datasets that practically require PPO, we minimize its subtle effects on the GCS by using the same algorithm hyper-parameters for training and testing and strictly set at the base case to reasonable values. We then adjust specific hyperparameters from the base case to view their effects experimentally.


We briefly explain some metrics and what they measure: 
\begin{itemize}
\item GCS: If training gradient is aligned more with true gradient, larger learning rates may be allowed. Furthermore,  \cite{batchnorm_madry} uses GCS as an approximation of the Hessian and smoothness of training landscape - having this oscillate too highly suggests a sharp minimizer, which is bad for generalization. 

\item Variance, Gradient Norm, and $\ell_{2}$ weight norm: The variance of the gradient estimation is dependent on both the batch-size as well as the Lipschitz smoothness of the policy gradient with respect to policy parameters, i.e. $\norm{\nabla_{\phi}R_{S}(\pi_{\phi}) - \nabla_{\phi}R_{S}(\pi_{\phi'})} \le L \cdot \norm{\phi - \phi'}$. Gradient Norm is a practical estimate of the Lipschitz constant between different total rewards, and $\ell_{2}$ is a rough estimate of the complexity of the policy.
\end{itemize}

\section{MDP's for Experimentation}
\cite{deeprl_matters,madrypolicygradient} establish deep RL experimentation is inherently noisy, and joint training only increases the variance of the policy gradient is increased further from sampling from different environments. The raw versions of ALE and Mujoco environments do not strongly follow distributional sampling of levels. We instead use both synthetic (RNN-MDP) and real (CoinRun) datasets, with policy gradient PPO as the default algorithm due to its reliability (hyperparameters in Appendix, \ref{hyper}).


\subsection{RNN-MDP}
To simulate non-linear dynamics for generalization, we fix an RNN to simulate $\mathcal{T}$. The RNN's (input, hidden state, output) correspond to the (action of a policy, underlying MDP state, $w, r$ observations and scalar rewards after being passed through $w,r$). The initial state will start from $s_{0}(\theta)$. Thus the the parameter $\theta$ will only be a seed to generate initial state. This setting is done in order to use a constant transition function, to guarantee that there always exists an optimal action for any state regardless of $\theta$. By allowing control over state transitions, we may study the effects of stochasticity in the environment, by adding Gaussian noise into the hidden state at each time, i.e. $s_{t}^{actual} = s_{t}^{raw} + \epsilon \mathcal{N}(0,1)$. We used precise gradient descent for joint training, in order for the policy to produce a precise policy gradient through the environment.

\subsubsection{Results}
(See Appendix \ref{fig:rnnmdp_stoch} and \ref{fig:rnnmdp_gamma} for enlarged graphs). 

\begin{figure}[H]
  \caption{Varying Stochasticities for RNN-MDP}
  \centering
    \includegraphics[scale = 0.12]{RNNMDP_stoch_gcs.pdf}
    \includegraphics[scale = 0.12]{RNNMDP_stoch_test.pdf}
\end{figure}

\begin{figure}[H]
  \caption{Varying $\gamma$ for nonstochastic and stochastic RNN-MDP}
  \centering
    \includegraphics[scale = 0.126]{RNN_MDP_gamma.pdf}

\end{figure}

We find that when adding stochasticity (e.g. random action stochasticity or sticky actions \cite{overfittingRL}) into actions the GCS increases, while the test loss decreases. This result is isolated from any other factors in RL, and thus shows that stochasticity aligns the policy gradient more to the true gradient. Since entropy and stochasticity may smoothen the loss landscape in RL \cite{entropy_regularization}, this suggests that entropy may be also therefore be affecting the direction of the gradient in particular ways impacting generalization.

Furthermore, when introducing stochasticity into the environment by perturbing the state transition randomly at each turn, we find that higher gamma values in reward produces better generalization, while in the deterministic setting without transition stochasticity, lower gamma value produce better generalization. Here, we see that entropy and stochasticity changes the monotonicity of $\gamma$ with respect to generalization - they have an interdependence. 


\subsection{Realistic MDP's - CoinRun}
\subsubsection{Differing Effects for Regularizers in RL }
We use CoinRun \cite{coinrun} as a procedurally generated MDP family for testing larger scale generalization. We see that steadily decreasing gradient cosine similarity (GCS) produces overall worse testing performance, and higher asymptotic GCS is correlated with good test performance. However, regularizers do not produce the exact same effects, but this is non-obvious: e.g. batchnorm changes the network weight norms while stochasticity does not, and stochasticity is heavily sensitive to batchsize.


We notice that normal training can have instability on its gradient cosine similarity (GCS) and thus smoothness - the exact time ($10^{3.8}$ timesteps) at which the GCS immediately rose, the test curve significantly dropped, leading to a poor test performance (see Appendix \ref{fig:gcs_unstable} for instability results).  
\begin{figure}[H]  
  \caption{GCS vs Various Modifications (normal training, batchnorm, batchnorm with stochasticity = 0.1, stochasticity = 0.1, data augmentation)} 
  \centering
    \includegraphics[scale = 0.126]{gcs_normal_stoch_batchnorm_dataaug.pdf}
    \label{fig:variousmods}
\end{figure} 

\begin{figure}[H]  
  \centering
    \includegraphics[scale = 0.127]{entropy.pdf}
    \includegraphics[scale = 0.127]{l2.pdf}
    \includegraphics[scale = 0.127]{config_gradnorm.pdf}
    \label{fig:variousmods_aux}
\end{figure} 
Data augmentation produces a constant non-zero GCS, as well as high asymptotic gradient norm, but does not significantly deviate network norm or entropy. This implies that data augmentation has a strong effect on the Lipschitz constant on the loss, but also does not allow the policy to converge, which is also consistent with the fact that its GCS does not converge to 0. 

Meanwhile, stochasticity leads to an overall better GCS consistent with \cite{entropy_regularization}, which correlates with the eventual higher test performance. Batchnorm reduces both the variance and the magnitude of the GCS consistent with \cite{batchnorm_madry}, while the addition of stochasticity with batch normalization increases the GCS overall slightly. Furthermore, batchnorm also has a similar effect to stochasticity on the policy entropy, but stochasticity does not change the $\ell_{2}$ norm of network weights, while batchnorm does. Batchnorm reduces the gradient norm, as does stochasticity when compared based on reward vs gradient norm.

We encourage the reader to view more results in Appendix \ref{fig:gcs_unstable}, \ref{fig:stoch_gradnorm}, which explores stochasticity's effects on gradient norm.

\subsubsection{Interdependence between Hyperparameters at a Larger Scale}
We investigate stochasticity's effects further, especially from batchsize. Both larger and smaller batchsizes generally \textit{benefit} batchnorm \cite{increasebatch}, and usually lower batchsizes improve generalization due to beneficial gradient noise \cite{largebatch} - we find that this is not the case for stochasticity. 

\begin{figure}[H] 
  \caption{GCS Instability with varying batchsize.}
  \centering
    \includegraphics[scale = 0.127]{gcs_unstable.pdf}
    \label{fig:stochbatch}
\end{figure} 
\begin{figure}[H]
  \centering
    \includegraphics[scale = 0.127]{l2_nminibatch_stoch01.pdf}
\end{figure} 
As shown above, action stochasticity (entropy regularization) naturally boosts GCS - however, extra boosts can be caused by unwanted high variance on the GCS (which can be exacerbated by poor choices of batchsize, suggesting existence of sharp minimizer) and actually lead to poorer test performance. While keeping stochasticity fixed to 0.1 (figure \ref{fig:stochbatch}) during training, the minibatch number (which inversely affects batchsize) has a strong effect on test performance and the weight norms, similar to SL. Surprisingly, higher batchsize (and thus less noise) produces significantly more variance on the GCS, also suggesting convergence on a sharp minimizer (i.e. high eigenvalue on the Hessian). 


Stochasticity also reduces the acceptable range of mini-batchnumber (figure \ref{fig:stoch_minibatch}), showing this parameter is important to RL generalization when using entropy bonuses. The batchsize normally provides a form of gradient noise which may help training - in the RL case this is translated to sampling individual policy gradient estimates from a mixture between the true policy gradient and the entropy added gradient. As expected, too much noise caused by low batchsize such as nminibatch = 64 produces negligible GCS. 

\begin{figure}[H] 
  \caption{Stochasticity vs NumMiniBatch} 
  \centering
    \includegraphics[scale = 0.13]{stoch_firstlast.pdf}
    \label{fig:stoch_minibatch}
\end{figure}

We provide more relationship analysis in Appedix \ref{fig:gammastoch_full}, testing relationships between stochasticity and $\gamma$ on CoinRun and CoinRun-Mazes (an RNN exploration test). 












